First Principles Heisenberg Models of 2D magnetic materials: The Importance of Quantum Corrections to the Exchange Coupling

Magnetic materials are typically described in terms of the Heisenberg model, which provides an accurate account of thermodynamic properties when combined with first principles calculations. This approach is usually based on an energy mapping between density functional theory and a classical Heisenberg model. However, for two-dimensional systems the eigenenergies of the Heisenberg model may differ significantly from the classical approximation, which leads to modified expressions for exchange parameters. Here we demonstrate that density functional theory yields local magnetic moments that are in accordance with strongly correlated anti-ferromagnetic eigenstates of the Heisenberg Hamiltonian. This implies that density functional theory provides a description of these states that conforms with the quantum mechanical eigenstates of the model. We then provide expressions for exchange parameters based on a proper eigenstate mapping to the Heisenberg model and find that they are typically reduced by 10 % compared to a classical analysis. Finally, we calculate the corrections to critical temperature for magnetic ordering for a previously predicted set of two-dimensional ferromagnetic insulators and find that the inclusion of quantum effects may reduce the predictions of critical temperatures by up to 7 %.

==> Antiferromagnetic%20quantum%20correction%20(updated%20version)/reply.tex <==
Dear editors

We wish to thank the referees for highly useful comments. They have certainly served to improve the manuscript. Below we provide our response to all the individual comments:



### Referee 1:

- A repeated “the” should be omitted from line 4 in the abstract.

Fixed.

- The sentence in the abstract section which starts from line 6 to line 9 is very
long and it should be separated into a few sentences.

The sentence has been broken up and is now more readable.

- In the last paragraph in the theory, the authors wrote:” in Exact DFT”! and later
on, they state “this could be, however, be a matter of luck and the value depends
rather strongly on the choice of functional”! First of all, I don’t think the DFT is
exact, so I would rather prefer omitting the word “exact”.

We have changed the wording to "Since the associated spin densities are in principle accurately described by DFT..." 

- The sentence after equation 9 is very confusing, the authors assumed that the
easy axis is along the z-direction, but in line 5 after the equation 9, the authors
state “which originates from the fact that the z-axis is not an easy axis”! in fact,
positive values of A means that the easy axis is along the z-direction, and one
can make the gap negative by choosing negative values for λ and keep the easy
axis along the z-direction. Could the authors explain this?

Yes, we have reformulated the entire discussion below Eq. 9 to explain that the spinwave gap only represents a physical quantity if it is positive. But that we can use the sign as a descriptor for broken rotational symmetry

- While reading the manuscript for the first time, I was wondering about not
including the Hubbard interaction! But I was surprised when the authors include
such interaction but they mentioned this in page 5! I think it will be much better if
the authors mention it in the introduction, or even in the theory.

Yes, we are now mentioning in the introduction that we compare DFT calculations with and without U.

- A reference should be added to the second paragraph after equation 9 when
authors state “We have previously shown that …”

Done.

- Last paragraph in (page 4, first column), in “Fig. III”, should be replaced by
Fig.3.

Done.

- Space should be placed between “and” and “associated”, this lies on page 5,
the second column in the discussion part (second paragraph, line 12).

Done.

9- Last paragraph, second line, “and” should be replaced by “an”.

Done.



### Referee 2:

- As the authors stressed, quantum correction is significant for small spins. This point should be emphasized earlier, for instance, right after (or around) the following sentence:
``However, in the case of 2D materials the anti-ferromagnetic configurations involved in the mapping are strongly correlated and are not necessarily well approximated by a classical configuration of the Heisenberg model."

Yes, we agree on this. We have added a comment that it is particularly important for low spin systems.

- In the 1st paragraph of Sec. II.A, the authors say, ``For a bipartite lattice there is a unique anti-ferromagnetic state where all sites are anti-aligned with neighboring sites". But this state is unique up to the SO(3) rotation in the spin space, right?

Right. We have added a comment that the configuration is only unique up to spin rotations.

- In the 2nd paragraph of Sec. II.A, it is said that there is a configuration in DFT corresponding to the NIM state, which shares the same symmetry with the Neel state. I suggest that the authors elaborate more on the nature of the state in the DFT side, as it is quite important to understand the actual procedure in the present approach.

We have elaborated a bit on this. It is tricky, however, since there is no direct link between the Kohn-Sham states and the correlated NIM state. Indeed, the magnetization density seems to be the only fingerprint, which is exactly what we are calculating.

- The authors should provide their definitions right after the place where $m_{AFM}/m_{FM}$ appears.

Yes, we have done that now and corrected our description of the magnetic moment (Eq. 5), which was written in an unclear way as pointed out by referee 3.

- Eq. (10) is based on the results obtained by classical Monte Carlo simulations of the model with $S \ne 1/2$. I wonder if the authors can include the case of $S=1/2$ by using quantum Monte Carlo simulations. As far as I understand, the model Eq. (8) on bipartite lattices such as square and honeycomb lattices do not suffer from a sign problem. (I have not checked but I think there must be some previous studies on this.)

Yes, that would certainly be highly useful. Even more if we could find quantum Monte Carlo simulations for S=1 for anisotropic 2D model. We have searched for this, but did not find anything useful. Our guess is that it is not an easy task to obtain the critical temperature from quantum Monte Carlo studies.

- For the reader's convenience, maybe the authors can write in the caption the meaning of the highlited materials with bold face.

Agree. We have done that now.

- In Abstract:
``for two-dimensional system the the eigenenergies ..."
-> ``for two-dimensional system the eigenenergies ..."

Done

- The last paragraph of Introduction:
``crucial influence on the prediction thermodynamic ..."
-> ``"crucial influence on the prediction of thermodynamic ...

Done

- 4 lines above Eq. (7)
``configurations has to be mapped ..."
-> ``configurations have to be mapped ..."
or ``configuration has to be mapped ..."

Done

- 2nd paragraph of Sec. III:
``In Fig. 1 we the display ..."
-> ``In Fig. 1 we display ..."

Done

- 3rd paragraph of Sec. III:
``In Fig. III we show ..."
- ``In Fig. 2 we show ..." (?)

Done 



### Referee 3:

- Moreover, the paper is also not written in a way that would make it a beneficial read for the wider condensed-matter community. For instance, it would have been interesting to compare the present approach to other techniques widely used in the community (such as direct determinations of the low-energy Hamiltonian using strong-coupling expansions or exact-diagonalization techniques, i.e., without mapping energies, or quantum chemistry calculations). The discussion is also restricted to systems for which the spin-orbit coupling is negligible and it remains unclear whether the method can be applied beyond this context.

Yes, that would certainly be highly interesting. However, we do not have any expertise in the methods mentioned and have not been able to find any good references that apply on 2D anisotropic Heisenberg Hamiltonians like the ones considered in the present work. If the referee can provide any reference for this it would be highly helpful.

- I therefore recommend to transfer the paper to a less selective journal.

Yes, the paper has been transferred to J. Phys.: Cond. Mat.

- The statement "for a ferromagnetic Heisenberg model (J>0) the NIM state can be regarded as the approximate eigenstate of highest energy" (p.2) is confusing. Which magnon state is meant here? If this state is not the ground state, why is the spin-wave spectrum still real? As this state is at very high energy, why is it of any relevance to the (low-energy) physics at all?

- It is the (frozen) magnon of highest energy situated at the Brillouin zone boundary. This is an eigenstate of the Heisenberg Hamiltonian (of highest energy) and is therefore real.

- I find it confusing that T_c and T_c^{Ising} have different units.

We agree. The T_c^{Ising} has been corrected so it now has the same units as T_C

- Why do the authors call m_{Abs} in Eq. (12) "magnetization density", although it is defined as an integral over the quantities m_\uparrow and m_\downarrow? I also couldn't find a definition for the latter quantities.

That was an error. Thanks for pointing this out. It has been corrected so it now reads "we have calculated the integral of the norm of the magnetization density..."

- Does "Fig. III" on p.4 mean "Fig. 2"?

Yes, that has been corrected now.

- The authors should also comment on effects beyond linear spin-wave theory, which may of relevance for small S.

We have added a sentence in the conclusion that methods beyond renormalized spin-wave theory (RPA) is required to deal with spin-1/2 systems. We have previously shown that the RPA breaks down for any value of S if anisotropy is strong. So applying spin-wave theory to the calculations of critical temperatures breaks down in RPA, which is why we are using classical Monte Carlo simulations. However, for the case of S=1/2 spin-wave theory (beyond RPA) or quantum Monte Carlo simulations seem to be the only way to go.



########## Additional changes:

We have added Eqs. 10-12 to make the energy mapping approach more explicit. We have also updated Fig. 2 and Table 1 with slightly updated numbers accordingly. 

Fig. 3 has been removed from the manuscript, since it did not convey much new information compared to Fig. 2

==> reply.tex <==
Dear editors

We wish to thank the referees for highly useful comments. They have certainly served to improve the manuscript. Below we provide our response to all the individual comments:



### Referee 1:

- A repeated “the” should be omitted from line 4 in the abstract.

Fixed.

- The sentence in the abstract section which starts from line 6 to line 9 is very
long and it should be separated into a few sentences.

The sentence has been broken up and is now more readable.

- In the last paragraph in the theory, the authors wrote:” in Exact DFT”! and later
on, they state “this could be, however, be a matter of luck and the value depends
rather strongly on the choice of functional”! First of all, I don’t think the DFT is
exact, so I would rather prefer omitting the word “exact”.

We have changed the wording to "Since the associated spin densities are in principle accurately described by DFT..." 

- The sentence after equation 9 is very confusing, the authors assumed that the
easy axis is along the z-direction, but in line 5 after the equation 9, the authors
state “which originates from the fact that the z-axis is not an easy axis”! in fact,
positive values of A means that the easy axis is along the z-direction, and one
can make the gap negative by choosing negative values for λ and keep the easy
axis along the z-direction. Could the authors explain this?

Yes, we have reformulated the entire discussion below Eq. 9 to explain that the spinwave gap only represents a physical quantity if it is positive. But that we can use the sign as a descriptor for broken rotational symmetry

- While reading the manuscript for the first time, I was wondering about not
including the Hubbard interaction! But I was surprised when the authors include
such interaction but they mentioned this in page 5! I think it will be much better if
the authors mention it in the introduction, or even in the theory.

Yes, we are now mentioning in the introduction that we compare DFT calculations with and without U.

- A reference should be added to the second paragraph after equation 9 when
authors state “We have previously shown that …”

Done.

- Last paragraph in (page 4, first column), in “Fig. III”, should be replaced by
Fig.3.

Done.

- Space should be placed between “and” and “associated”, this lies on page 5,
the second column in the discussion part (second paragraph, line 12).

Done.

9- Last paragraph, second line, “and” should be replaced by “an”.

Done.



### Referee 2:

- As the authors stressed, quantum correction is significant for small spins. This point should be emphasized earlier, for instance, right after (or around) the following sentence:
``However, in the case of 2D materials the anti-ferromagnetic configurations involved in the mapping are strongly correlated and are not necessarily well approximated by a classical configuration of the Heisenberg model."

Yes, we agree on this. We have added a comment that it is particularly important for low spin systems.

- In the 1st paragraph of Sec. II.A, the authors say, ``For a bipartite lattice there is a unique anti-ferromagnetic state where all sites are anti-aligned with neighboring sites". But this state is unique up to the SO(3) rotation in the spin space, right?

Right. We have added a comment that the configuration is only unique up to spin rotations.

- In the 2nd paragraph of Sec. II.A, it is said that there is a configuration in DFT corresponding to the NIM state, which shares the same symmetry with the Neel state. I suggest that the authors elaborate more on the nature of the state in the DFT side, as it is quite important to understand the actual procedure in the present approach.

We have elaborated a bit on this. It is tricky, however, since there is no direct link between the Kohn-Sham states and the correlated NIM state. Indeed, the magnetization density seems to be the only fingerprint, which is exactly what we are calculating.

- The authors should provide their definitions right after the place where $m_{AFM}/m_{FM}$ appears.

Yes, we have done that now and corrected our description of the magnetic moment (Eq. 5), which was written in an unclear way as pointed out by referee 3.

- Eq. (10) is based on the results obtained by classical Monte Carlo simulations of the model with $S \ne 1/2$. I wonder if the authors can include the case of $S=1/2$ by using quantum Monte Carlo simulations. As far as I understand, the model Eq. (8) on bipartite lattices such as square and honeycomb lattices do not suffer from a sign problem. (I have not checked but I think there must be some previous studies on this.)

Yes, that would certainly be highly useful. Even more if we could find quantum Monte Carlo simulations for S=1 for anisotropic 2D model. We have searched for this, but did not find anything useful. Our guess is that it is not an easy task to obtain the critical temperature from quantum Monte Carlo studies.

- For the reader's convenience, maybe the authors can write in the caption the meaning of the highlited materials with bold face.

Agree. We have done that now.

- In Abstract:
``for two-dimensional system the the eigenenergies ..."
-> ``for two-dimensional system the eigenenergies ..."

Done

- The last paragraph of Introduction:
``crucial influence on the prediction thermodynamic ..."
-> ``"crucial influence on the prediction of thermodynamic ...

Done

- 4 lines above Eq. (7)
``configurations has to be mapped ..."
-> ``configurations have to be mapped ..."
or ``configuration has to be mapped ..."

Done

- 2nd paragraph of Sec. III:
``In Fig. 1 we the display ..."
-> ``In Fig. 1 we display ..."

Done

- 3rd paragraph of Sec. III:
``In Fig. III we show ..."
- ``In Fig. 2 we show ..." (?)

Done 



### Referee 3:

- Moreover, the paper is also not written in a way that would make it a beneficial read for the wider condensed-matter community. For instance, it would have been interesting to compare the present approach to other techniques widely used in the community (such as direct determinations of the low-energy Hamiltonian using strong-coupling expansions or exact-diagonalization techniques, i.e., without mapping energies, or quantum chemistry calculations). The discussion is also restricted to systems for which the spin-orbit coupling is negligible and it remains unclear whether the method can be applied beyond this context.

Yes, that would certainly be highly interesting. However, we do not have any expertise in the methods mentioned and have not been able to find any good references that apply on 2D anisotropic Heisenberg Hamiltonians like the ones considered in the present work. If the referee can provide any reference for this it would be highly helpful.

- I therefore recommend to transfer the paper to a less selective journal.

Yes, the paper has been transferred to J. Phys.: Cond. Mat.

- The statement "for a ferromagnetic Heisenberg model (J>0) the NIM state can be regarded as the approximate eigenstate of highest energy" (p.2) is confusing. Which magnon state is meant here? If this state is not the ground state, why is the spin-wave spectrum still real? As this state is at very high energy, why is it of any relevance to the (low-energy) physics at all?

- It is the (frozen) magnon of highest energy situated at the Brillouin zone boundary. This is an eigenstate of the Heisenberg Hamiltonian (of highest energy) and is therefore real.

- I find it confusing that T_c and T_c^{Ising} have different units.

We agree. The T_c^{Ising} has been corrected so it now has the same units as T_C

- Why do the authors call m_{Abs} in Eq. (12) "magnetization density", although it is defined as an integral over the quantities m_\uparrow and m_\downarrow? I also couldn't find a definition for the latter quantities.

That was an error. Thanks for pointing this out. It has been corrected so it now reads "we have calculated the integral of the norm of the magnetization density..."

- Does "Fig. III" on p.4 mean "Fig. 2"?

Yes, that has been corrected now.

- The authors should also comment on effects beyond linear spin-wave theory, which may of relevance for small S.

We have added a sentence in the conclusion that methods beyond renormalized spin-wave theory (RPA) is required to deal with spin-1/2 systems. We have previously shown that the RPA breaks down for any value of S if anisotropy is strong. So applying spin-wave theory to the calculations of critical temperatures breaks down in RPA, which is why we are using classical Monte Carlo simulations. However, for the case of S=1/2 spin-wave theory (beyond RPA) or quantum Monte Carlo simulations seem to be the only way to go.



########## Additional changes:

We have added Eqs. 10-12 to make the energy mapping approach more explicit. We have also updated Fig. 2 and Table 1 with slightly updated numbers accordingly. 

Fig. 3 has been removed from the manuscript, since it did not convey much new information compared to Fig. 2
